Generalizable Neural Human Renderer

While recent advancements in animatable human rendering have achieved remarkable results, they require test-time optimization for each subject which can be a significant limitation for real-world applications. To address this, we tackle the challenging task of learning a Generalizable Neural Human Renderer (GNH), a novel method for rendering animatable humans from monocular video without any test-time optimization. Our core method focuses on transferring appearance information from the input video to the output image plane by utilizing explicit body priors and multi-view geometry. To render the subject in the intended pose, we utilize a straightforward CNN-based image renderer, foregoing the more common ray-sampling or rasterizing-based rendering modules. Our GNH achieves remarkable generalizable, photorealistic rendering with unseen subjects with a three-stage process. We quantitatively and qualitatively demonstrate that GNH significantly surpasses current state-of-the-art methods, notably achieving a 31.3% improvement in LPIPS.

==> tabs/feature_ablation.tex <==
% \begin{wraptable}{R}{0.5\linewidth}
% \centering
% \resizebox{0.5\columnwidth}{!}{
% \begin{tabular}{lcccc}
%     \Xhline{3\arrayrulewidth}
%          & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & Avg. $\downarrow$ \\ \hline
%          $ \phi_\text{refine} (\phi_\text{dino}(I))$ &  &  & \\
%          $ \phi_\text{fine} (I)$ &  &  & \\
%          $ \phi_\text{fine} (I) \oplus \phi_\text{refine} (\phi_\text{dino}(I))$ &  &  & \\\hline 
%     \end{tabular}}
%     \caption{some caption for first table} 
%     \label{tab:featenc_ablation}
% \end{wraptable}

==> tabs/supp_ablation.tex <==
\begin{table}[tb]
    \centering
    \captionsetup{aboveskip=0pt}\captionsetup{belowskip=0pt}
    \caption{Additional Ablations and comparisons. Our final model is underlined.}
    \scalebox{0.87}{
    \begin{tabular}{llccccc}
    \Xhline{3\arrayrulewidth}
                    \multicolumn{1}{c}{Experiment}              & \multicolumn{1}{c}{Method}  & PSNR$\uparrow$ & SSIM$\uparrow$ & LPIPS$\downarrow$ & \multicolumn{2}{c}{Avg. $\downarrow$}  \\ \hline \hline
        \multirow{4}{*}{Feat dim of $\Phi_\text{multi\_frame}$} & 32 & 27.26 & 0.962  & 42.64 & 24.93 & (+0.) \\
                                    & 64 & 27.30 & 0.962  & 43.46 & 25.04 & (+5.99) \\
                                    & 128 & 27.45 & 0.962 & 41.77 & 24.41 & (+0.35) \\
                                    & \ul{256} & 27.24 & 0.963 & 42.00 & 24.81  &  (+0.86) \\ \hline 
        \multirow{3}{*}{Depth of $\Phi_\text{multi\_frame}$}& 2 & 27.32 & 0.961 &  41.91 & 24.56 & (+0.61) \\
                                    & 3 & 26.45 & 0.956  & 56.71 & 29.94 & (+5.99) \\
                                     & \ul{4} & 24.84 & 0.954 & 51.79 & 33.25 &  (+9.30)\\ 
        \hline
    \end{tabular}}
    \label{tab:supp_ablation}
\end{table}
